SketchFill: Sketch-Guided Code Generation for Imputing Derived Missing Values

Missing value is a critical issue in data science, significantly impacting the reliability of analyses and predictions. Missing value imputation (MVI) is a longstanding problem because it highly relies on domain knowledge. Large language models (LLMs) have emerged as a promising tool for data cleaning, including MVI for tabular data, offering advanced capabilities for understanding and generating content. However, despite their promise, existing LLM techniques such as in-context learning and Chain-of-Thought (CoT) often fall short in guiding LLMs to perform complex reasoning for MVI, particularly when imputing derived missing values, which require mathematical formulas and data relationships across rows and columns. This gap underscores the need for further advancements in LLM methodologies to enhance their reasoning capabilities for more reliable imputation outcomes. To fill this gap, we propose SketchFill, a novel sketch-based method to guide LLMs in generating accurate formulas to impute missing numerical values. Our experimental results demonstrate that SketchFill significantly outperforms state-of-the-art methods, achieving 56.2% higher accuracy than CoT-based methods and 78.8% higher accuracy than MetaGPT. This sets a new standard for automated data cleaning and advances the field of MVI for numerical values.

==> sections/impact.tex <==
\section{Broader Impact}
\label{sec:impact}
% \stitle{Checklist 10. Broader Impacts} 
LLMs are increasingly applied in assistance of manual workload. Our work, \sys, has shown considerable promise in avenue for enhancing the accuracy and efficiency of imputing missing value, especially in the scenario where understanding the formulaic relation within data and contexts is important, however, it also may generate incorrect answers for imputation when the formulas extracted by \sys are inconsistent with the ground truth formulaic relation of dataset. We believe that when applying this research to practice, the imputation function needs to be reviewed and approved by human experts. 
%and further research can focus on multi-step formula extraction.

==> sections/limitation.tex <==
%!TEX root = ../main.tex
\section{Limitation}
\label{sec:limitation}
% This paper has explored and achieved outstanding accuracy in formulaic relation variables, which formula is single-step within rows or columns. 
% more subjective judgment
This paper has explored and outperformed the other 6 methods in our experiments in formulaic relation variables, which formula is single-step within rows or columns.
However, specific to the formula that contains multiple steps for computation, \sys may extract the incorrect formula, such as RSI8. In this case, the incorrect formula can be distinguished and amended based on the result of the Summarizer under human review. Approaches such as MetaGPT can also be alternatively applied. \sys has also observed a lack of performance in the dataset that contains fabricated data or data that is inconsistent with the ground truth formula. Future work should consider techniques that enhance the multi-step reasoning of formula construction and fabricated data detection in DMVI tasks.
